Can LLMs Extract Frame-Semantic Arguments?

Frame-semantic parsing is a critical task in natural language understanding, yet the ability of large language models (LLMs) to extract frame-semantic arguments remains underexplored. This paper presents a comprehensive evaluation of LLMs on frame-semantic argument identification, analyzing the impact of input representation formats, model architectures, and generalization to unseen and out-of-domain samples. Our experiments, spanning models from 0.5B to 78B parameters, reveal that JSON-based representations significantly enhance performance, and while larger models generally perform better, smaller models can achieve competitive results through fine-tuning. We also introduce a novel approach to frame identification leveraging predicted frame elements, achieving state-of-the-art performance on ambiguous targets. Despite strong generalization capabilities, our analysis finds that LLMs still struggle with out-of-domain data.

==> figures/per_frame_boxplot.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/per_frame_boxplot.png}
  
  \caption{\label{fig:frame-boxplot} Comparison of the distribution of F1 scores across all frames for each model.}
\end{figure}

==> sections/generated_prompt_examples.tex <==
Your task is to analyze the given sentence and identify all the frame elements associated with the Abandonment frame. A frame in linguistics is a schematic representation of a situation involving various participants, props, and other conceptual roles, known as frame elements. The Abandonment frame involves an Agent who leaves behind a Theme, effectively rendering it no longer within their control or normal security as their property.

Below are some details regarding the Abandonment frame:

1. **Frame Definition**: An Agent leaves behind a Theme, effectively rendering it no longer within their control or of the normal security as one's property.

2. **Frame Elements**:
    - **Agent (Core)**: The person who acts to leave behind the Theme.
    - **Theme (Core)**: The entity that is relinquished to no one from the Agent's possession.
    - **Place (Peripheral)**: The location where the Agent gives up the Theme.
    - **Time (Peripheral)**: When the Agent gives up the Theme.
    - **Manner (Peripheral)**: The style in which the Agent gives up the Theme.
    - **Duration (Peripheral)**: For what expanse of time the Agent has given up the Theme.
    - **Explanation (Extra-Thematic)**: A proposition from which the act of abandonment logically follows.
    - **Depictive (Extra-Thematic)**: Describes the Agent during the abandoning event.
    - **Degree (Peripheral)**: The extent to which the Agent leaves the Theme behind.
    - **Means (Peripheral)**: An action performed by the Agent that accomplishes the action.
    - **Purpose (Peripheral)**: The purpose for which the Agent abandons the Theme.
    - **Event_description (Extra-Thematic)**: A description of the event as a whole.

3. **Examples**:
    - "Carolyn abandoned her car and jumped on a red double decker bus." 
      - Frame Elements: {"Agent": "Carolyn", "Theme": "her car"}
    - "Jamie Hill, prosecuting, said Stevenson and a friend took a Nova car from North Skelton and abandoned it in Nottingham."
      - Frame Elements: {"Agent": "Stevenson and a friend", "Theme": "it", "Place": "in Nottingham"}

Using this information, identify the relevant frame elements in the following input sentence. Your response should be structured in JSON format with frame elements as keys and the specific text references from the sentence as values. Ensure every frame element is present as a key, with an empty string if not applicable.

Input Sentence: {input_sentence}

Output the frame elements in JSON format, exemplified as:
```
{
    "Agent": "text",
    "Theme": "text",
    "Place": "text",
    "Time": "text",
    "Manner": "text",
    "Duration": "text",
    "Explanation": "text",
    "Depictive": "text",
    "Degree": "text",
    "Means": "text",
    "Purpose": "text",
    "Event_description": "text"
}
```


--------------------------------------------------------------------------------

To identify all the frame elements associated with the "Activity_stop" frame in a given sentence, use the information provided below. Based on the sentence structure and context, determine the relevant frame elements and their corresponding text in the sentence. Ensure that the output is formatted in JSON, with the frame elements as keys and the corresponding text from the sentence as values.

Here are the details about the "Activity_stop" frame:
- **Frame_Definition**: An Agent ceases an Activity without completing it.
- **Frame_Elements**:
  - **Agent (Core)**: Identifies the Agent that stops the Activity.
  - **Activity (Core-Unexpressed)**: Identifies the Activity that the Agent stops.
  - **Purpose (Extra-Thematic)**: Identifies the Purpose for which an Agent stopped the Activity.
  - **Place (Peripheral)**: Identifies the Place where the Agent stops the Activity.
  - **Time (Peripheral)**: Identifies the Time when the Agent stops the Activity.
  - **Depictive (Extra-Thematic)**: For Depictive phrases describing the actor or undergoer.
  - **Manner (Peripheral)**: Identifies the Manner in which the Agent stops the Activity.
  - **Result (Extra-Thematic)**: Identifies the Result of the stopped Activity.
  - **Duration (Peripheral)**: Length of Time during which the Activity is stopped.
  - **Means (Extra-Thematic)**: Identifies the Means by which the Agent stops the Activity.
  - **Co-timed_event (Extra-Thematic)**: Identifies the last Co-timed_event of the stopped Activity.
  - **Degree (Peripheral)**: Describes the completeness of stopping.
  - **Frequency (Extra-Thematic)**: Number of times an event occurs. 
  - **Containing_event (Extra-Thematic)**: Event during which the Agent stops the Activity.
  - **Circumstances (Extra-Thematic)**: Describes the state of the world at the time of the event.
  - **Re-encoding (Extra-Thematic)**: Presents the frame as a part of a larger conceptualization.
  - **Explanation (Extra-Thematic)**: Reason the Agent stops the Activity.
  - **Event_description (Extra-Thematic)**: Describes the clause as a whole.
  - **Particular_iteration (Extra-Thematic)**: Part of an iterated series of events.

**Task**: Given the sentence: "{input_sentence}", identify and extract the relevant frame elements based on the "Activity_stop" frame. Format and provide the output in JSON as shown below:

```json
{
    "frame_element_1": "text",
    "frame_element_2": "text",
    ...
}
```


--------------------------------------------------------------------------------



To identify all the frame elements associated with the "Adducing" frame in a given sentence, follow the steps below. Frame semantics is a theory that describes the understanding of a word's meaning based on the conceptual frame it evokes. Each frame involves various participants and conceptual roles known as frame elements.

**Frame: Adducing**
- **Definition**: A Speaker mentions a Specified_entity filling a Role, thereby providing information which supports a point of the Speaker.

**Core Frame Elements:**
- **Speaker**: The person who specifies the Role to be filled by the Specified_entity.
- **Specified_entity**: The entity that the Speaker identifies as filling a particular Role.
- **Role**: A slot in a particular event or relation whose filler the Speaker identifies.

**Peripheral Frame Elements:**
- **Addressee**: The person to whom the Speaker identifies the filler of a Role.
- **Manner**: Description of how the act is performed.
- **Means**: The act whereby the Speaker makes a statement.
- **Medium**: The physical entity or channel used by the Speaker to transmit the statement.
- **Time**: The time when the statement is made.
- **Place**: Where the statement takes place.
- **Purpose**: What the Speaker intends to accomplish by adducing the Specified_entity.
- **Explanation**: The reason for which the Speaker comes to the conclusion about the Specified_entity.
- **Containing_event**: The context or event in which the adducing occurs.
- **Event_description**: Descriptions related to the entire clause.
- **Frequency**: How often the event occurs.
- **Circumstances**: The context or conditions under which the adducing takes place.
- **Depictive**: The state or condition of the Speaker during the statement.

**Instructions:**
- Analyze the provided sentence to identify words or phrases that correspond to each of the possible frame elements listed above.
- Provide a json output listing the recognized frame elements and their corresponding text from the sentence.

Here is your input sentence for analysis:

"{input_sentence}"

**Output format example:**

```json
{
    "Specified_entity": "text",
    "Speaker": "text",
    "Role": "text",
    "Manner": "text",
    ...
}
```

Please ensure the json output lists only the elements present in the sentence, leaving absent elements out.

==> sections/titan_prompt.tex <==
You will be acting as an intelligent entity that gives an instruction to another large language model.

Your task is to generate a prompt for another large language model such that it identifies all the frame elements
associated with a particular frame in a given sentence.

You are free to generate a prompt that involves as much information as you see fit for the other large language
model. You can include examples, definitions, etc. as you see fit.

In the generated prompt, have a pair of curly braces with "input\_sentence" where 
the input sentwnce can be injected. Also include the instruction that the final output should be in json
format and should look like :


    frame\_element\_1 : text,
    frame\_element\_2 : text,
    ...


Here frame\_element\_1, frame\_element\_2, etc are the name of the frame elements.

Your output should be the prompt only.

Here is some information about "Frame semantics":
\{frame\_semantics\_definition\}

Here is some information about "frame":
\{frames\_definition\}

Here is some information about "Frame elements":
\{frame\_elements\_definition\}

The frame that you will be working with is called \{frame\_name\}
Here are details about the frame \{frame\_name\} with its definition, frame elements, the definitions of its frame elements, some examples of sentences that evoke the frame and some annotated examples that show frame elements
in the sentence.

\{frame\_details\}

==> tables/arg-id.tex <==
%   Model                   | Representation        | Precision (near)  | Recall    | F1    | Accuracy  | Cost
% ----------------------------------------------------------------------------------------------------
% ============= W/ Exemplar =============
% GPT-4o-mini (0 temp)      | JSON-complete         | 0.356 (0.475)     | 0.577     | 0.440 | 0.282     | 3$
% GPT-4o-mini (1 temp)      | JSON-complete         | 0.349 (0.469)     | 0.569     | 0.433 | 0.276     | 3$
% GPT-4o-mini (0 temp)      | JSON-complete-cot     | 0.103 (0.112)     | 0.567     | 0.175 | 0.096     | 3$
% GPT-4o-mini (0 temp)      | JSON-exist            | 0.416 (0.530)     | 0.543     | 0.471 | 0.308     | 3$
% GPT-4o-mini (0 temp)      | JSON-exist-cot        | 0.413 (0.529)     | 0.562     | 0.476 | 0.312     | 3$
% GPT-4o-mini (0 temp)      | XML-tag               | 0.318 (0.442)     | 0.368     | 0.342 | 0.206     | 3$
% GPT-4o-mini (1 temp)      | XML-tag               | 0.308 (0.431)     | 0.359     | 0.332 | 0.199     | 3$
% GPT-4o-mini (1 temp)      | XML-tag               | 0.310 (0.432)     | 0.361     | 0.333 | 0.200     | 3$
% GPT-4o-mini (0 temp)      | Markdown              | 0.xxx (0.xxx)     | 0.xxx     | 0.xxx | 0.xxx     | 3$
% GPT-4o (0 temp)           | JSON-exist            | 0.550 (0.660)     | 0.642     | 0.592 | 0.420     | $$


% KID                       | -                     | 0.741             | 0.773     | 0.756 | -         | -
% AGED                      | -                     | 0.757             | 0.776     | 0.762 | -         | -
% Ai, Tu (2024)             | -                     | 0.764             | 0.777     | 0.771 | -         | -


% ============= W/o Exemplar ============

% GPT-4o-mini-smallhqft     | JSON-exist            | 0.605 (0.697)     | 0.699     | 0.649 | 0.480     | 5$
% GPT-4o-mini-smallft       | JSON-exist            | 0.717 (0.824)     | 0.675     | 0.696 | 0.533     | 5$
% GPT-4o-mini-ft            | JSON-exist            | 0.774 (0.856)     | 0.762     | 0.768 | 0.624     | 25$

% GPT-4o-finetune           | JSON-exist            | 0.??? (0.???)     | 0.???     | 0.??? | 0.???     | 300$
% GPT-4o-finetune-small     | JSON-exist            | 0.??? (0.???)     | 0.???     | 0.??? | 0.???     | 30$

% Llama 3.2-3B-ft           | json-exist            | 0.717 (0.841)     | 0.691     | 0.704 | 0.543     | Free
% Llama 3.1-8B-4bit-ft      | json-exist            | 0.736 (0.850)     | 0.711     | 0.724 | 0.567     | Free


% Lin et al (2021)          | -                     | -                 | -         | 0.721 | -         | -
% AGED                      | -                     | 0.750             | 0.752     | 0.751 | -         | -
% Ai, Tu (2024)             | -                     | 0.756             | 0.753     | 0.755 | -         | -



==> tables/full-fe-table.tex <==
\begin{table*}
    \centering
    \begin{tabularx}{\textwidth}{Xlcccc}
        \hline
        Model & Representation & Precision & Recall & F1 & Accuracy \\ 
        \hline
        GPT-4o-mini     & JSON-complete     & 0.356 & 0.577 & 0.440 & 0.282 \\ 
        GPT-4o-mini     & JSON-exist        & 0.416 & 0.543 & 0.471 & 0.308 \\ 
        GPT-4o-mini     & XML-tag           & 0.318 & 0.368 & 0.342 & 0.206 \\ 
        GPT-4o-mini     & Markdown          & 0.xxx & 0.xxx & 0.xxx & 0.xxx \\ 
        GPT-4o          & JSON-exist        & 0.550 & 0.642 & 0.592 & 0.420 \\ 
        \hline
        KID             & -                 & 0.741 & 0.773 & 0.756 & - \\ 
        AGED            & -                 & 0.757 & 0.776 & 0.762 & - \\ 
        Ai, Tu (2024)   & -                 & 0.764 & 0.777 & 0.771 & - \\ 
        \hline
        
        \hline
    \end{tabularx}
    \caption{Performance metrics for different models and representations.}
    \label{tab:model_representation_performance}
\end{table*}



% Llama 3.2-3B-ft           | json-exist            | 0.717 (0.841)     | 0.691     | 0.704 | 0.543     | Free
% Llama 3.1-8B-4bit-ft      | json-exist            | 0.736 (0.850)     | 0.711     | 0.724 | 0.567     | Free
